Formalized $q$-series: The Rogers-Ramanujan Identities and Beyond

The theory of $q$-series and basic hypergeometric series plays a crucial role at the intersection of combinatorics, number theory, and representation theory. From the classical partition identities of Euler and Jacobi to modern developments in class field theory, vertex operator algebras, and the Monstrous Moonshine conjecture, $q$-series provide the analytic framework for a wide range of profound applications. In this paper, we discuss the formalization of this theory in the Lean proof assistant, a process that requires careful design of scalable and versatile structures to reconcile formal algebraic identities with analytic convergence properties. We address these foundational challenges by focusing on the construction of $q$-Pochhammer symbols, $q$-binomial coefficients, Bailey's Lemma and similar primitives. To demonstrate the utility of this work, we provide fully verified proofs of the Jacobi Triple Product formula and the celebrated Rogers-Ramanujan identities, which serve as both historical and technical benchmarks for the field. This work establishes a rigorous computational foundation for the future formalization of mock theta functions, modular forms, and the diverse algebraic structures that underpin their applications across mathematics and physics. AxiomProver was used to produce the formalizations in this paper.

==> lstlean.tex <==
% lstlean.tex --- Lean language definition for the listings package.
% Well-formed version: the entire definition is a single, properly
% brace-balanced argument to \lstdefinelanguage, so it is absorbed by
% the parser instead of leaking into the document body.

\lstdefinelanguage{lean}{%
  mathescape=false,
  texcl=false,
  morekeywords=[1]{%
    import, prelude, protected, private, noncomputable, definition, meta,
    renaming, hiding, parameter, parameters, begin, constant, constants,
    lemma, variable, variables, theory, print, theorem, example, open, as,
    universe, universes, alias, help, precedence, reserve, declare_trace,
    add_key_equivalence, match, infix, infixl, infixr, notation, postfix,
    prefix, instance, eval, reduce, check, coinductive, mutual, def,
    run_cmd, section, namespace, end, this, suppose, using, using_well_founded,
    structure, inductive, class, attribute, abbreviation, extends, include,
    omit, do, by, hiding, exit, calc, set_option, next, then, else, from,
    let, if, in, at, with, deriving, fun, assume, show, have, suffices,
    obtain, replace, generalizing},
  morekeywords=[2]{Sort, Type, Prop},
  morekeywords=[3]{%
    assumption, apply, intro, intros, allGoals, generalize, clear, revert,
    done, exact, refine, repeat, cases, rewrite, rw, simp, simpa, simp_all,
    contradiction, constructor, injection, induction, norm_num, norm_num1,
    tauto, itauto, field_simp, linarith, nlinarith, ring, ring_nf, omega,
    decide, trivial, rfl, sorry, admit, unfold, dsimp, change, subst, use,
    existsi, split, left, right, ext, funext, congr, convert, exact?,
    apply?, simp?, aesop, gcongr, positivity, bound, grind},
  literate=%
    {α}{{\ensuremath{\alpha}}}1
    {β}{{\ensuremath{\beta}}}1
    {γ}{{\ensuremath{\gamma}}}1
    {δ}{{\ensuremath{\delta}}}1
    {ε}{{\ensuremath{\varepsilon}}}1
    {ζ}{{\ensuremath{\zeta}}}1
    {η}{{\ensuremath{\eta}}}1
    {θ}{{\ensuremath{\theta}}}1
    {ι}{{\ensuremath{\iota}}}1
    {κ}{{\ensuremath{\kappa}}}1
    {μ}{{\ensuremath{\mu}}}1
    {ν}{{\ensuremath{\nu}}}1
    {ξ}{{\ensuremath{\xi}}}1
    {π}{{\ensuremath{\pi}}}1
    {ρ}{{\ensuremath{\rho}}}1
    {σ}{{\ensuremath{\sigma}}}1
    {τ}{{\ensuremath{\tau}}}1
    {φ}{{\ensuremath{\varphi}}}1
    {χ}{{\ensuremath{\chi}}}1
    {ψ}{{\ensuremath{\psi}}}1
    {ω}{{\ensuremath{\omega}}}1
    {Γ}{{\ensuremath{\Gamma}}}1
    {Δ}{{\ensuremath{\Delta}}}1
    {Θ}{{\ensuremath{\Theta}}}1
    {Λ}{{\ensuremath{\Lambda}}}1
    {Σ}{{\ensuremath{\Sigma}}}1
    {Φ}{{\ensuremath{\Phi}}}1
    {Ξ}{{\ensuremath{\Xi}}}1
    {Ψ}{{\ensuremath{\Psi}}}1
    {Ω}{{\ensuremath{\Omega}}}1
    {ℵ}{{\ensuremath{\aleph}}}1
    {≤}{{\ensuremath{\leq}}}1
    {≥}{{\ensuremath{\geq}}}1
    {≠}{{\ensuremath{\neq}}}1
    {≈}{{\ensuremath{\approx}}}1
    {≡}{{\ensuremath{\equiv}}}1
    {≃}{{\ensuremath{\simeq}}}1
    {∂}{{\ensuremath{\partial}}}1
    {∆}{{\ensuremath{\Delta}}}1
    {∫}{{\ensuremath{\int}}}1
    {Π}{{\ensuremath{\Pi}}}1
    {⊥}{{\ensuremath{\bot}}}1
    {∞}{{\ensuremath{\infty}}}1
    {∓}{{\ensuremath{\mp}}}1
    {±}{{\ensuremath{\pm}}}1
    {×}{{\ensuremath{\times}}}1
    {⊕}{{\ensuremath{\oplus}}}1
    {⊗}{{\ensuremath{\otimes}}}1
    {⊞}{{\ensuremath{\boxplus}}}1
    {∇}{{\ensuremath{\nabla}}}1
    {√}{{\ensuremath{\surd}}}1
    {·}{{\ensuremath{\cdot}}}1
    {•}{{\ensuremath{\bullet}}}1
    {∘}{{\ensuremath{\circ}}}1
    {⬝}{{\ensuremath{\cdot}}}1
    {▸}{{\ensuremath{\triangleright}}}1
    {∧}{{\ensuremath{\wedge}}}1
    {∨}{{\ensuremath{\vee}}}1
    {¬}{{\ensuremath{\neg}}}1
    {⊢}{{\ensuremath{\vdash}}}1
    {⟨}{{\ensuremath{\langle}}}1
    {⟩}{{\ensuremath{\rangle}}}1
    {↦}{{\ensuremath{\mapsto}}}1
    {←}{{\ensuremath{\leftarrow}}}1
    {→}{{\ensuremath{\rightarrow}}}1
    {↔}{{\ensuremath{\leftrightarrow}}}1
    {⇒}{{\ensuremath{\Rightarrow}}}1
    {⟹}{{\ensuremath{\Longrightarrow}}}1
    {⇐}{{\ensuremath{\Leftarrow}}}1
    {⟸}{{\ensuremath{\Longleftarrow}}}1
    {∩}{{\ensuremath{\cap}}}1
    {∪}{{\ensuremath{\cup}}}1
    {⊂}{{\ensuremath{\subset}}}1
    {⊆}{{\ensuremath{\subseteq}}}1
    {⊄}{{\ensuremath{\not\subset}}}1
    {⊈}{{\ensuremath{\nsubseteq}}}1
    {⊃}{{\ensuremath{\supset}}}1
    {⊇}{{\ensuremath{\supseteq}}}1
    {⊅}{{\ensuremath{\not\supset}}}1
    {⊉}{{\ensuremath{\nsupseteq}}}1
    {∈}{{\ensuremath{\in}}}1
    {∉}{{\ensuremath{\notin}}}1
    {∋}{{\ensuremath{\ni}}}1
    {∌}{{\ensuremath{\not\ni}}}1
    {∅}{{\ensuremath{\emptyset}}}1
    {∖}{{\ensuremath{\setminus}}}1
    {†}{{\ensuremath{\dagger}}}1
    {⌞}{{\ensuremath{\llcorner}}}1
    {⌟}{{\ensuremath{\lrcorner}}}1
    {⦃}{{\ensuremath{\lbrace}}}1
    {⦄}{{\ensuremath{\rbrace}}}1
    {‖}{{\ensuremath{\|}}}1
    {ℕ}{{\ensuremath{\mathbb{N}}}}1
    {ℤ}{{\ensuremath{\mathbb{Z}}}}1
    {ℝ}{{\ensuremath{\mathbb{R}}}}1
    {ℚ}{{\ensuremath{\mathbb{Q}}}}1
    {ℂ}{{\ensuremath{\mathbb{C}}}}1
    {ℍ}{{\ensuremath{\mathbb{H}}}}1
    {↑}{{\ensuremath{\uparrow}}}1
    {↓}{{\ensuremath{\downarrow}}}1
    {∀}{{\ensuremath{\forall}}}1
    {∃}{{\ensuremath{\exists}}}1
    {λ}{{\ensuremath{\lambda}}}1
    {₀}{{\ensuremath{_0}}}1
    {₁}{{\ensuremath{_1}}}1
    {₂}{{\ensuremath{_2}}}1
    {₃}{{\ensuremath{_3}}}1
    {₄}{{\ensuremath{_4}}}1
    {₅}{{\ensuremath{_5}}}1
    {₆}{{\ensuremath{_6}}}1
    {₇}{{\ensuremath{_7}}}1
    {₈}{{\ensuremath{_8}}}1
    {₉}{{\ensuremath{_9}}}1
    {ᵢ}{{\ensuremath{_i}}}1
    {ⱼ}{{\ensuremath{_j}}}1
    {ₐ}{{\ensuremath{_a}}}1
    {ₙ}{{\ensuremath{_n}}}1
    {ₘ}{{\ensuremath{_m}}}1
    {ₚ}{{\ensuremath{_p}}}1
    {¹}{{\ensuremath{^1}}}1
    {⁻}{{\ensuremath{^-}}}1
    {ˣ}{{\ensuremath{^x}}}1
    {∑}{{\ensuremath{\textstyle\sum}}}1
    {∏}{{\ensuremath{\textstyle\prod}}}1
    {:=}{{:=}}2
    {==}{{==}}2
    {++}{{++}}2
    {**}{{**}}2,
  morecomment=[s]{/-}{-/},
  morecomment=[l]{--},
  showstringspaces=false,
  keepspaces=true,
  morestring=[b]",
  tabsize=2,
  extendedchars=true,
  sensitive=true,
  breaklines=true,
  breakatwhitespace=true,
  captionpos=b,
  columns=fullflexible%
}

